Medical Image Segmentation with Belief Function Theory and Deep Learning

Deep learning has shown promising contributions in medical image segmentation with powerful learning and feature representation abilities. However, it has limitations for reasoning with and combining imperfect (imprecise, uncertain, and partial) information. In this thesis, we study medical image segmentation approaches with belief function theory and deep learning, specifically focusing on information modeling and fusion based on uncertain evidence. First, we review existing belief function theory-based medical image segmentation methods and discuss their advantages and challenges. Second, we present a semi-supervised medical image segmentation framework to decrease the uncertainty caused by the lack of annotations with evidential segmentation and evidence fusion. Third, we compare two evidential classifiers, evidential neural network and radial basis function network, and show the effectiveness of belief function theory in uncertainty quantification; we use the two evidential classifiers with deep neural networks to construct deep evidential models for lymphoma segmentation. Fourth, we present a multimodal medical image fusion framework taking into account the reliability of each MR image source when performing different segmentation tasks using mass functions and contextual discounting.

==> externs/classicthesis-config.tex <==
% !TEX encoding = UTF-8 Unicode
\RequirePackage{microtype} % character protruding and other micro-typography stuff
\RequirePackage{booktabs} % for better rules in tables
\RequirePackage{textcase} % for \MakeTextUppercase
% Other configurations 
\microtypesetup{expansion=false}
\DeclareRobustCommand{\spacedallcaps}[1]{\textls[160]
			{\MakeTextUppercase{#1}}}
\DeclareRobustCommand{\spacedlowsmallcaps}[1]{\textls[80]
			{\scshape\MakeTextLowercase{#1}}}
			
% ********************************************************************
% Pretty right note of paragraph
% ********************************************************************
% Graffiti as in GKP's book "Concrete Mathematics"
% thanks to Lorenzo Pantieri and Enrico Gregorio
\def\graffito@setup{%
%   \slshape\footnotesize% this was due to \slhape in above book
   \itshape\footnotesize\leavevmode\color{Black}%
   \parindent=0pt 
   \lineskip=0pt 
   \lineskiplimit=0pt %
   \tolerance=2
   \hyphenpenalty=300 
   \exhyphenpenalty=300%
   \doublehyphendemerits=1000%
   \finalhyphendemerits=\doublehyphendemerits
 }

\let\oldmarginpar\marginpar
% always add optional parameter, make it empty by default
\renewcommand{\marginpar}[2][]{
   % optional parameter empty, in all normal document calls
   \if\relax\detokenize{#1}\relax
   \oldmarginpar[\graffito@setup\raggedleft\hspace{0pt}#2]
      {\graffito@setup\raggedright\hspace{0pt}#2}%
   %two parameters, let them use their styling
   \else
      \oldmarginpar[#1]{#2}%
   \fi%
}
\let\graffito\marginpar

% *************************************************************
% Font Stuff
% *************************************************************

\PassOptionsToPackage{osf,sc}{mathpazo}%
% Palatino with real small caps and old style figures
\RequirePackage{mathpazo} 
\linespread{1.05} % a bit more for Palatino
\PassOptionsToPackage{scaled=0.85}{beramono}%
\RequirePackage{beramono}%
\PassOptionsToPackage{euler-digits}{eulervm}%
\RequirePackage{eulervm} % Euler math fonts


% ********************************************************************
% footnotes setup
% ********************************************************************
% \ifdefined\deffootnote
%     % KOMA-command, footnotemark not superscripted at the bottom
%     \deffootnote{0em}{0em}{\thefootnotemark\hspace*{.5em}}%
%     \message{Using KOMA-command "deffootnote" for footnote setup}%
% \else
     \PassOptionsToPackage{flushmargin}{footmisc}%
     \RequirePackage{footmisc}%
     \setlength{\footnotemargin}{-.5em}%
% \fi

% The idea is progressively does not use the classicthesis style 
%\PassOptionsToPackage{
%  nochapters=false,
%  % print version information on the bottom of the pages
%  drafting=false, %-----DONE----
%  % the left column of the toc will be aligned (no indentation)
%  tocaligned=false, 
%  % page numbers in ToC flushed right
%  dottedtoc=false,  
%  % use part division
%  parts=true,       
%  % use AMS Euler for chapter font (otherwise Palatino)
%  eulerchapternumbers=false, 
%  % chaper headers will have line above and beneath 
%  linedheaders=false, 
%  % numbering per chapter for all floats (i.e.,Figure 1.1)
%  floatperchapter=false,
%  % load listings package and setup LoL
%  listings=false,    
%  % setup for preloaded subfig package
%  subfig=false,      
%  % use awesome Euler fonts for mathematical formulae (only with pdfLaTeX)
%  eulermath=false,  
%}{classicthesis}
%
%\usepackage{classicthesis}


==> externs/doctoralthesis.tex <==
% !TEX encoding = UTF-8 Unicode
% The idea is progressively does not use the Johannes Böttcher style 
%------------------------------------------------------------------
% Default variables used to remove code not necessary 
%------------------------------------------------------------------
% consistentlayout=true

%------------------------------------------------------------------
%% Generic commands used whole style
%------------------------------------------------------------------
% Addchap provides unnumbered chapters with an entry in
% the table of contents as well as an updated header
\ProvideDocumentCommand{\addchap}{ s o m }{%
	\chapter*{#3}%
	\markboth{}{}%
	\IfBooleanTF{#1}{%
	}{%
		\IfNoValueTF{#2}{%
			\addchaptertocentry{#3}%
			\markboth{\MakeMarkcase{#3}}{\MakeMarkcase{#3}}%
		}{%
			\addchaptertocentry{#2}%
			\markboth{\MakeMarkcase{#2}}{\MakeMarkcase{#2}}%
		}%
	}%
}%

% If the liststotoc option has been passed to the class, 
% add the lists to the table of contents
\ifbool{liststotoc}{
	\patchcmd{\listoftables}{\@starttoc{lot}}{%
		\addchaptertocentry{\listtablename}\@starttoc{lot}%
	}{}{}%
	\patchcmd{\listoffigures}{\@starttoc{lof}}{%
		\addchaptertocentry{\listfigurename}\@starttoc{lof}%
	}{}{}%
}

%------------------------------------------------------------------
%% DEFINE CUSTOM THESIS INFORMATION COMMANDS
%------------------------------------------------------------------
\NewDocumentCommand{\thesistitle} { o m }{%
 \IfValueTF{#1}{\def\shorttitle{#1}}{\def\shorttitle{#2}}%
 \def\@title{#2}%
 \def\ttitle{#2}%
}
\DeclareDocumentCommand{\author}{m}{
	\newcommand{\authorname}{#1}
%	\renewcommand{\@author}{#1} % @salmuz
}	
\NewDocumentCommand{\authorweb}{m}{\newcommand{\authweb}{#1}}
\NewDocumentCommand{\supervisor}{m}{\newcommand{\supname}{#1}}
\NewDocumentCommand{\supervisorweb}{m}{\newcommand{\supweb}{#1}}
\NewDocumentCommand{\examiner}{m}{\newcommand{\examname}{#1}}
\NewDocumentCommand{\degree}{m}{\newcommand{\degreename}{#1}}
\NewDocumentCommand{\addresses}{m}{\newcommand{\addressname}{#1}}
\NewDocumentCommand{\university}{m}{\newcommand{\univname}{#1}}
\NewDocumentCommand{\department}{m}{\newcommand{\deptname}{#1}}
\NewDocumentCommand{\group}{m}{\newcommand{\groupname}{#1}}
\NewDocumentCommand{\faculty}{m}{\newcommand{\facname}{#1}}
\NewDocumentCommand{\subject}{m}{\newcommand{\subjectname}{#1}}
\NewDocumentCommand{\keywords}{m}{\newcommand{\keywordnames}{#1}}
\newcommand{\checktoopen}{
% New command to move content to the next page which
% prints to the next odd page if twosided mode is active  
	\if@openright\cleardoublepage\else\clearpage\fi
	\ifdef{\phantomsection}{\phantomsection}{}
	% The \phantomsection command is necessary for 
	% hyperref to jump to the correct page
}
\NewDocumentCommand{\bhrule}{}{\typeout{--------------------}}
\NewDocumentCommand{\tttypeout}{m}{\bhrule\typeout{\space #1}\bhrule}
% The depth to which the document sections are printed
% to the table of contents
\setcounter{tocdepth}{3} 
\ProvideDocumentCommand{\addchaptertocentry}{ m }{%
	\addcontentsline{toc}{chapter}{#1}%
}

%------------------------------------------------------------------
%% DECLARATION PAGE DESIGN
%------------------------------------------------------------------
\newcommand{\authorshipname}{Declaration of Authorship}
% Declaration of Authorship text for English countries
\providecaptionname{american,
	australian,british,
	canadian,english,newzealand,UKenglish,
	USenglish}{\authorshipname}{Declaration of Authorship} 
% Declaration of Authorship text for Germanic countries
\providecaptionname{german,ngerman,austrian,
	naustrian}{\authorshipname}{Eidesstattliche Erkl\"arung} 

\DeclareDocumentEnvironment{declaration}{}{
		\checktoopen
		\tttypeout{\authorshipname}
		\thispagestyle{plain}
		\null\vfil
		{\noindent\huge\bfseries\authorshipname\par\vspace{10pt}}
	}{}




%------------------------------------------------------------------
%% DECLARATION PAGE DESIGN
%------------------------------------------------------------------
\newcommand{\publicationname}{List of Publications}
% Declaration of Authorship text for English countries
\providecaptionname{american,
	australian,british,
	canadian,english,newzealand,UKenglish,
	USenglish}{\publicationname}{List of Publications} 
% Declaration of Authorship text for Germanic countries
\providecaptionname{german,ngerman,austrian,
	naustrian}{\publicationname}{List of Publications} 

\DeclareDocumentEnvironment{publication}{}{
		\checktoopen
		\tttypeout{\publicationname}
		\thispagestyle{plain}
		\null\vfil
		{\noindent\huge\bfseries\publicationname\par\vspace{10pt}}
	}{}


%------------------------------------------------------------------
%	ABSTRACT PAGE DESIGN
%------------------------------------------------------------------
\DeclareDocumentCommand{\abstractauthorfont}{}{}
\DeclareDocumentCommand{\abstracttitlefont}{}{}
\newcommand{\byname}{by}
\newcommand{\abstractname}{Abstract}

\providecaptionname{german,ngerman,austrian,
	naustrian}{\byname}{von}
\providecaptionname{american,australian,
	british,canadian,english,newzealand,
	UKenglish,USenglish}{\byname}{by}
	
\DeclareDocumentEnvironment{abstract}{ O{\null\vfill} }{
	\checktoopen
	\tttypeout{\abstractname}
	#1%added to be able to have abstract more than one page long
	\thispagestyle{plain}
	\begin{center}
		% University name in capitals
		{\normalsize \MakeUppercase{\univname} \par}
		\bigskip
		{\huge\textit{\abstractname} \par}
		\bigskip
		{\normalsize \groupname \par}% Faculty name
%		{\normalsize \deptname \par}% Department name
		\bigskip
		{\normalsize \degreename\par}% Degree name
		\bigskip
		{\normalsize\bfseries \@title \par}% Thesis title
		\medskip
		{\normalsize \byname{} \authorname \par}% Author name
		\bigskip
	\end{center}
}{
	\vfill\null
}
%------------------------------------------------------------------
%	ACKNOWLEDGEMENTS PAGE DESIGN
%------------------------------------------------------------------
\newcommand{\acknowledgementname}{Acknowledgements}
% Acknowledgement text for English countries
\providecaptionname{american,australian,
	british,canadian,english,newzealand,
	UKenglish,USenglish}{\acknowledgementname}{Acknowledgements} 

% Acknowledgement text for Germanic countries
\providecaptionname{german,ngerman,austrian,
	naustrian}{\acknowledgementname}{Danksagung} 

\DeclareDocumentEnvironment{acknowledgements}{}{%
	\checktoopen
	\tttypeout{\acknowledgementname}
	\thispagestyle{plain}
	\begin{center}{\huge\textit{\acknowledgementname}\par}\end{center}
}{
	\vfil\vfil\null
}


%------------------------------------------------------------------
%	ACKNOWLEDGEMENTS PAGE DESIGN
%------------------------------------------------------------------
\newcommand{\introductionname}{Introduction}
% Acknowledgement text for English countries
\providecaptionname{english,british,
		american}{\introductionname}{Introduction}%{Acknowledgements} 

% Acknowledgement text for Germanic countries
\NewDocumentEnvironment{introduction}{  }{%
	%%%\ifbool{nolistspace}{\begingroup\singlespacing}{}
	\ifbool{liststotoc}{\addchap{\introductionname}}{\addchap*{\introductionname}}


	%%%\ifbool{nolistspace}{\endgroup}{}
}


%------------------------------------------------------------------
%	CONSTANTS AND OTHERS PAGE DESIGN
%-----------------------------------------------------------------
\newcommand{\constantsname}{List of Notations}
\providecaptionname{english,british,american}{\constantsname}{List of Notations}
%\providecaptionname{ngerman,german,austrian,naustrian}{\constantsname}{Listenschreibweise}
\NewDocumentEnvironment{constants}{ m }{%
	\ifbool{liststotoc}{\addchap{\constantsname}}{\addchap*{\constantsname}}
	\begin{longtable}{#1}
	}{
	\end{longtable}
	% Don't count this table as one of the document tables
	\addtocounter{table}{-1}
}

%------------------------------------------------------------------
%	ABBREVIATIONS PAGE DESIGN
%------------------------------------------------------------------
\newcommand{\abbrevname}{List of Abbreviations}
\providecaptionname{english,british,
		american}{\abbrevname}{List of Abbreviations}
\providecaptionname{ngerman,german,austrian,
		naustrian}{\abbrevname}{Abk\"urzungsverzeichnis}
		
\NewDocumentEnvironment{abbreviations}{ m }{
	\ifbool{liststotoc}{\addchap{\abbrevname}}{\addchap*{\abbrevname}}
	\begin{longtable}{#1}
	}{
	\end{longtable}
	% Don't count this table as one of the document tables
	\addtocounter{table}{-1}
	%%%\ifbool{nolistspace}{\endgroup}{}
}
%------------------------------------------------------------------
%	SYMBOLS PAGE DESIGN
%------------------------------------------------------------------
\newcommand{\symbolsname}{List of Symbols}
\providecaptionname{english,british,
	american}{\symbolsname}{List of Symbols}
\providecaptionname{ngerman,german,austrian,
	naustrian}{\symbolsname}{Symbolverzeichnis}

\NewDocumentEnvironment{symbols}{ m }{%
	%%%\ifbool{nolistspace}{\begingroup\singlespacing}{}
	\ifbool{liststotoc}{\addchap{\symbolsname}}{\addchap*{\symbolsname}}
	\begin{longtable}{#1}
	}{
	\end{longtable}
	% Don't count this table as one of the document tables
	\addtocounter{table}{-1}
	%%%\ifbool{nolistspace}{\endgroup}{}
}
%------------------------------------------------------------------
%	DEDICATION PAGE DESIGN
%------------------------------------------------------------------
\newcommand\dedicatory[1]{
	\checktoopen
	\tttypeout{Dedicatory}
	\null\vfil
	\thispagestyle{plain}
	\begin{center}{\Large\slshape #1}\end{center}
	\vfil\null
}


==> externs/salmuz.tex <==
% !TEX encoding = UTF-8 Unicode
%------------------------------------------------------------------
% custom bibliography format
% [WARNING] Loading before hyperref package (backref option)

\usepackage[backend=bibtex,
		    style=authoryear,
            bibstyle=authoryear,
            citestyle=authoryear,
            natbib=true,
            maxbibnames=100, % max name to show bibliography
            maxcitenames=1, % max name to show cite command
            backref=true, % load hyerref before else it does not work
            abbreviate=true]{biblatex}

\DeclareCiteCommand{\cite}[\mkbibbrackets]
  {\usebibmacro{prenote}}
  {\usebibmacro{citeindex}%
   \printtext[bibhyperref]{\usebibmacro{cite}}}
  {\multicitedelim}
  {\usebibmacro{postnote}}
  
\DeclareCiteCommand{\citeauthor}
  {\boolfalse{citetracker}%
   \boolfalse{pagetracker}%
   \usebibmacro{prenote}}
  {\ifciteindex{\indexnames{labelname}}{}%
   \printtext[bibhyperref]{\printnames{labelname}}}
  {\multicitedelim}
  {\usebibmacro{postnote}}
  
\DeclareCiteCommand{\citeauthors}
	{\defcounter{maxnames}{99}%
	 \defcounter{minnames}{99}%
	 \defcounter{uniquename}{2}%
	 \boolfalse{citetracker}%
     \boolfalse{pagetracker}%
	 \usebibmacro{prenote}}
	{\ifciteindex{\indexnames{labelname}}{}%
	 \printtext[bibhyperref]{\printnames{labelname}}
	}
	{\multicitedelim}
	{\usebibmacro{postnote}}
    
%\DeclareCiteCommand{\fullcite}
%  {\usebibmacro{prenote}}
%  {
%   \usebibmacro{citeindex}%
%   \printtext[bibhyperref]{
%   		\usebibmacro{author}\usebibmacro{date}.\usebibmacro{title}
%   }
%  }
%  {\multicitedelim}
%  {\usebibmacro{postnote}}
  
%  {\usebibmacro{prenote}}
%  {\usedriver
%     {\DeclareNameAlias{sortname}{default}%
%      %\DeclareNameWrapperAlias{sortname}{coloursortname}%
%      \xpatchbibmacro{date+extradate}
%        {\printtext[parens]}
%        {}%\printtext[colourparens]}
%        {}
%        {}}
%     {\thefield{entrytype}}}
%  {\multicitedelim}
%  {\usebibmacro{postnote}}
\newcommand{\myfullciteunpublished}[2]{
	\citeauthor{#1}~(\citeyear{#1}).~
	\citetitle{#1}.~\emph{(#2)}
}
\newcommand{\myfullcite}[1]{
	\citeauthor{#1}~(\citeyear{#1}).~
	\citetitle{#1}.~In:~
	\citefield{#1}{booktitle}.} 

\DeclareCiteCommand{\citetitle}
  {\boolfalse{citetracker}%
   \boolfalse{pagetracker}%
   \usebibmacro{prenote}}
  {\ifciteindex
     {\indexfield{indextitle}}
     {}%
   	\printtext[bibhyperref]{
   		\printfield[citetitle]{labeltitle}}
  }{\multicitedelim}
  {\usebibmacro{postnote}}
  
\DefineBibliographyStrings{english}{%
    backrefpage  = {\textcolor{blue}{cited on p.}}, % for single page number
    backrefpages = {\textcolor{blue}{cited on pp.}} % for multiple page numbers
}


%------------------------------------------------------------------
% new packages maths tools 
%\usepackage{newpxmath}
\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{bm}
\usepackage{mathrsfs}
\usepackage{amsmath}
\usepackage{amssymb}
\allowdisplaybreaks

\usepackage{bbm} % indicator matrix 1
%
\newenvironment{psmallmatrix}
  {\left(\begin{smallmatrix}}
  {\end{smallmatrix}\right)}

%------------------------------------------------------------------
% Generic packages
\usepackage{hyperref}
\hypersetup{
	pdfpagemode={UseOutlines},
    colorlinks=true,
    linkcolor=mdtRed,
    urlcolor=MidnightBlue,
    citecolor=blue,
	bookmarksopen=true,
	bookmarksopenlevel=0,
	pdfstartview={FitV},
	unicode,
	breaklinks=true,
%	linktocpage=true
}

\usepackage{float}
\usepackage{subfig}
\captionsetup[subfigure]{
   margin=0cm,
   font=small,
   format=plain,
   labelfont={bf,up},
   textfont={up}
}

%------------------------------------------------------------------
% new commands cross-ref with name in capital first letter
\newcommand{\figureref}[1]{Figure \ref{#1}}
\newcommand{\equationref}[1]{Equation \eqref{#1}}
\newcommand{\definitionref}[1]{Definition \ref{#1}}
\newcommand{\sectionref}[1]{Section \ref{#1}}
\newcommand{\tableref}[1]{Table \ref{#1}}
\newcommand{\defintionref}[1]{Definition \ref{#1}}

%------------------------------------------------------------------
% theorem definitions
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{case}{Case}
\newtheorem{proof}{Proof}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}

%------------------------------------------------------------------
% changer format Roman chapter to arabic for contents/list of figures/list of tables
%\renewcommand{\thechapter}{\Roman{chapter}} 
%\renewcommand{\thesection}{\arabic{chapter}.\arabic{section}}
%\renewcommand{\thesubsection}{\arabic{chapter}.\arabic{section}.\arabic{subsection}}
%\renewcommand{\theequation}{\arabic{chapter}.\arabic{equation}}
%\renewcommand{\thefigure}{\arabic{chapter}.\arabic{figure}}
%\renewcommand{\thetable}{\arabic{chapter}.\arabic{table}}

%------------------------------------------------------------------
%https://tex.stackexchange.com/questions/26042/how-can-i-get-a-line-break-in-a-theorem-headline
%Line break in a theorem headline
\makeatletter
\renewcommand*{\@opargbegintheorem}[3]{\trivlist
      \item[\hskip \labelsep{\bfseries #1\ #2}] \textbf{(#3)}\ \itshape}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% WARNING: load scrlayer-scrpage before titlesec package.     %%%
%%% WARNING: \pagestyle{plain} -> remove headers/footers.       %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage[automark]{scrlayer-scrpage} % (KOMA Script)
%------------------------------------------------------------------
% Headers and Footers information
%------------------------------------------------------------------
\clearpairofpagestyles
\let\MakeMarkcase\spacedlowsmallcaps
\renewcommand{\sectionmark}[1]{
	\markboth{\thesection\enspace\spacedlowsmallcaps{#1}}
		{\thesection\enspace\spacedlowsmallcaps{#1}}
}
\renewcommand{\subsectionmark}[1]{
	\markboth{\thesubsection\enspace\spacedlowsmallcaps{#1}}
		{\thesubsection\enspace\spacedlowsmallcaps{#1}}
}
\lehead{\mbox{\llap{\small\pagemark\kern2em}\headmark\hfil}}
\rohead{\mbox{\hfil{\headmark}\rlap{\small\kern2em\pagemark}}}
\renewcommand{\headfont}{\small}
% hack to get the content headlines right (thanks, Lorenzo!)
\def\toc@heading{
	\chapter*{\contentsname}
    \@mkboth{\spacedlowsmallcaps{\contentsname}}
    		{\spacedlowsmallcaps{\contentsname}}
} 


% Clean chapter quotations
\newcommand{\hugequote}{%
	{\fontsize{75}{80}\selectfont%
	\hspace*{-.575em}\color{gray}%
	\includegraphics[scale=0.5]{images/hds/virgule.jpg}%
	\vskip -.4em}% 
}

\newcommand{\cleanchapterquote}[3]{%
	\begin{minipage}{\textwidth}%
		\begin{flushright}
			\begin{minipage}{.65\textwidth}%
				\begin{flushleft}
					{\hugequote}\textit{#1}
				\end{flushleft}
	    		\begin{flushright}
    				--- \textbf{#2} \\
    				#3
		    	\end{flushright}
		    \end{minipage}%
		\end{flushright}
	\end{minipage}%
	\bigskip
}
%
% Clean Quotation environment
\newenvironment{thesis_quotation}%
	{%
	\begin{minipage}{\textwidth}%
		\begin{flushright}
			\begin{minipage}{.95\textwidth}%
	}%
	{%
			\end{minipage}%
		\end{flushright}
	\end{minipage}%
	}%
%


==> front-back-matter/abbreviations.tex <==
% Include a list of abbreviations (a table of two columns)
%\addchaptertocentry{\abbrevname}
\begin{large}
\begin{abbreviations}{l@{\hskip 0.8in}l}
	%\textbf{AI} & \textsc{\textbf{A}rtificial \textbf{I}ntelligence} \\[1.5mm]
	%\textbf{ML} & \textsc{\textbf{M}achine \textbf{L}earning} \\[1.5mm]
	%\textbf{DL} & \textsc{\textbf{D}eep \textbf{L}earning} \\[1.5mm]
	\textbf{DNN} & \textsc{\textbf{D}eep \textbf{N}eural \textbf{N}etworks} \\[1.5mm]
	\textbf{CNN} & \textsc{\textbf{C}onvolutional \textbf{N}eural \textbf{N}etworks} \\[1.5mm]
	\textbf{BFT} & \textsc{\textbf{B}elief \textbf{F}unction \textbf{T}heory} \\[1.5mm]
	
	\textbf{CT} &\textsc{\textbf{C}omputed \textbf{T}omography} \\[1.5mm]
	\textbf{PET} &\textsc{\textbf{P}ositron \textbf{E}mission \textbf{T}omography}\\[1.5mm]
	\textbf{MRI} &\textsc{\textbf{M}agnetic \textbf{R}esonance \textbf{I}maging}\\[1.5mm]
	\textbf{FDG} &\textsc{\textbf{F}luoro \textbf{D}eoxy \textbf{G}lucose }\\[1.5mm]
	\textbf{TE} &\textsc{\textbf{T}ime \textbf{E}cho }\\[1.5mm]
	\textbf{RT} &\textsc{\textbf{R}epetition \textbf{T}ime }\\[1.5mm]
	\textbf{FLAIR} &\textsc{\textbf{FL}uid-\textbf{A}ttenuated \textbf{I}nversion \textbf{R}ecovery }\\[1.5mm]
	\textbf{FDG} &\textsc{\textbf{F}fluoro \textbf{D}eoxy\textbf{G}lucose }\\[1.5mm]
	
	
	\textbf{ROI} &\textsc{\textbf{R}egion  \textbf{O}f  \textbf{I}nterest}\\[1.5mm]
	\textbf{TP} &\textsc{\textbf{T}rue \textbf{P}ositive}\\[1.5mm]
	\textbf{TF} &\textsc{\textbf{T}rue \textbf{N}egative}\\[1.5mm]	
	\textbf{FP} &\textsc{\textbf{F}alse \textbf{P}ositive}\\[1.5mm]	
	\textbf{FN} &\textsc{\textbf{F}alse \textbf{N}egative}\\[1.5mm]	
	\textbf{HD} &\textsc{\textbf{H}ausdorff \textbf{D}istance}\\[1.5mm]	
	
	\textbf{ED} &\textsc{\textbf{ED}ema}\\[1.5mm]
	\textbf{ET} &\textsc{\textbf{E}nhancing \textbf{T}umor}\\[1.5mm]
	\textbf{NRC/NET} &\textsc{\textbf{N}ecrotic  \textbf{C}ore/\textbf{N}one \textbf{E}nhancing  \textbf{T}umor}\\[1.5mm]	

	
	\textbf{BBA} &\textsc{\textbf{B}asic \textbf{B}elief \textbf{A}ssignment}\\[1.5mm]
	\textbf{DM} &\textsc{\textbf{D}ecision  \textbf{M}aking}\\[1.5mm]
	\textbf{EKNN} &\textsc{\textbf{E}vidential \textbf{K}-\textbf{N}earest \textbf{N}eighbor}\\[1.5mm]	
	\textbf{BFOD} &\textsc{\textbf{B}inary \textbf{F}rames \textbf{O}f \textbf{D}iscernment}\\[1.5mm]		
	\textbf{ENN} &\textsc{\textbf{E}vidential \textbf{N}eural \textbf{N}etwork}\\[1.5mm]
	\textbf{RBF} &\textsc{\textbf{R}adial \textbf{B}asis \textbf{F}unction}\\[1.5mm]
	\textbf{FCM} &\textsc{\textbf{F}uzzy  {C}-\textbf{M}eans}\\[1.5mm]	
	\textbf{ECM} &\textsc{\textbf{E}vidential  {C}-\textbf{M}eans}\\[1.5mm]	
	\textbf{GD} &\textsc{\textbf{G}aussian  \textbf{D}istribution}\\[1.5mm]	
	\textbf{MV} &\textsc{\textbf{M}ebership  \textbf{V}alue}\\[1.5mm]	
	
	\textbf{BraTs} &\textsc{\textbf{B}rain \textbf{T}umor \textbf{S}egmentation}\\[1.5mm]
	
	\textbf{ECE} &\textsc{\textbf{E}xpected \textbf{C}alibartion \textbf{E}rror}\\[1.5mm]
	\textbf{MCD} &\textsc{\textbf{M}onte-\textbf{C}arlo \textbf{D}ropout}\\[1.5mm]	
	\textbf{FE} &\textsc{\textbf{F}eature \textbf{E}xtraction }\\[1.5mm]	
	\textbf{SE} &\textsc{\textbf{E}vidential \textbf{S}egmentation}\\[1.5mm]
	\textbf{MMEF} &\textsc{\textbf{M}ulti{M}odal \textbf{E}vidence \textbf{F}usion}\\[1.5mm]
	
	\textbf{CPU} &\textsc{\textbf{G}raphics \textbf{P}rocessor \textbf{U}nit}\\[1.5mm]
	\textbf{FLOPs} &\textsc{\textbf{FL}ating point \textbf{OP}erations}\\[1.5mm]
\end{abbreviations}
\end{large}


==> front-back-matter/authorship.tex <==
%------------------------------------------------------------------------
%	DECLARATION PAGE
%------------------------------------------------------------------------

\begin{declaration}
	% Add the declaration to the table of contents
	\addchaptertocentry{\authorshipname} 
	\noindent I, \authorname, declare that this thesis titled, \enquote{\ttitle} and the work presented in it are my own. I confirm that:
	\begin{itemize} 
		\item This work was done wholly or mainly while in candidature for a research degree at this University.
		\item Where any part of this thesis has previously been submitted for a degree or any other qualification at this University or any other institution, this has been clearly stated.
		\item Where I have consulted the published work of others, this is always clearly attributed.
		\item Where I have quoted from the work of others, the source is always given. With the exception of such quotations, this thesis is entirely my own work.
		\item I have acknowledged all main sources of help.
		\item Where the thesis is based on work done by myself jointly with others, I have made clear exactly what was done by others and what I have contributed myself.\\
	\end{itemize}
 
	\noindent Signed:\\
	\rule[0.5em]{25em}{0.5pt} % This prints a line for the signature
 
	\noindent Date:\\
	\rule[0.5em]{25em}{0.5pt} % This prints a line to write the date
\end{declaration}
\cleardoublepage

==> front-back-matter/dedication.tex <==
\dedicatory{To my parents}




==> front-back-matter/list-figures.tex <==
%---------------------------------------------------------------
%	LIST OF CONTENTS/FIGURES/TABLES PAGES
%---------------------------------------------------------------

%\tableofcontents % Prints the main table of contents

%\listoffigures % Prints the list of figures

%\listoftables % Prints the list of tables


==> front-back-matter/list-notations.tex <==
% The list of notations maths
\begin{constants}{ll}\label{tab:notations} 
\scshape{\Large Symbols} & \scshape{\Large Description}\\

\mbox{}\\[2mm]
\textsc{\large Data related notations} &\\[2mm]
$\mathbf{X}$ & Object space\\
$x$ & Object belonging to $\mathbf{X}$\\
$\mathbf{Y}$ & Target space\\
$y$ & Target belonging to $\mathbf{Y}$\\
$\hat{y}$ & Precise output prediction \\

\mbox{}\\[2mm]
\textsc{\large Probability and statistics} & \\[2mm]
$P(A)$ & Unconditional probability of event $A$\\
$P(A \mid B)$ & Conditional probability of event $A$ \\ & knowing event $B$\\
$\mathbb{P}$ & Probability measure\\
$\mathscr{P}$ & Set of probabilities\\
$\theta$ & Unknown parameters\\

\mbox{}\\[2mm]
\textsc{\large Conformal Prediction} & \\[2mm]
$\lbag z_1, \dots, \dots, z_n \rbag$ & Bag of examples\\
$\mathbf{Z}^{tr}$ & Proper training set\\
$\mathbf{Z}^{cal}$ & Calibration set\\
$\mathbf{Z}^{ts}$ & Test set\\
$\epsilon$ & Significance level\\
$\Gamma$ & Confidence predictor\\

\mbox{}\\[2mm]
\textsc{\large Mathematic and other notations} & \\[2mm]
$(\cdot)^T$ & Transpose operator \\
$(\cdot)^{-1}$ & Inverse operator \\
$\norm{\cdot}$ & Euclidian norm \\
$E$ & Ellipsoid\\
$B_m$ & Unit ball\\

\end{constants}



==> front-back-matter/list-tables.tex <==
%---------------------------------------------------------------
%	LIST OF CONTENTS/FIGURES/TABLES PAGES
%---------------------------------------------------------------

%\tableofcontents % Prints the main table of contents

%\listoffigures % Prints the list of figures

%\listoftables % Prints the list of tables


==> front-back-matter/quotation.tex <==
%\usepackage{arabtex}
%\vspace*{0.2\textheight}
%\begin{arabtext}
%\noindent\enquote{\itshape على قدر أهل العلم تأتي العزائم العزائم\\
%\hspace*{3pt}و تأتي على قدر الكرام المكارم\\
%\hspace*{3pt}وتعظم في عين الصغير صغارها\\
%\hspace*{3pt}وتصغر في عين العظيم العظائم}
%\end{arabtext}
%\bigbreak
%\bigbreak

\noindent\enquote{\itshape Il y a des hommes qui luttent un jour et ils sont bons,\\
\hspace*{3pt}d’autres luttent un an et ils sont meilleurs,\\
\hspace*{3pt}il y a ceux qui luttent pendant de nombreuses années et ils sont très bons,\\
\hspace*{3pt}mais il y a ceux qui luttent toute leur vie et ceux-là sont \textbf{les indispensables.}}
\bigbreak
\bigbreak

\noindent\enquote{\itshape There are men that fight one day and are good,\\
\hspace*{3pt}others fight one year and they’re better,\\
\hspace*{3pt}and there are those who fight many years and are very good,\\
\hspace*{3pt}but there are the ones who fight their whole lives and those are \textbf{the indispensable one}}
\bigbreak
\bigbreak

\noindent\enquote{\itshape Hay hombres que luchan un día y son buenos.\\
\hspace*{3pt}Hay otros que luchan un año y son mejores.\\
\hspace*{3pt}Hay quienes luchan muchos años y son muy buenos.\\
\hspace*{3pt}Pero hay los que luchan toda la vida. Esos son los \textbf{imprescindibles.}}

\bigbreak
\hfill Bertolt Brecht 

==> resources/mlcbr/eg_Iprob_loss_tree.tex <==
\newcommand{\exptwoeg}[3]{\underline{\mathbb{E}}_{Y_{\{#1\}}|\newinstance}\left[ \ell_H(\cdot, \overline{a}_\mathcal{I}) \middle| Y_{\{#2\}}\!=\!#3\right]}
\newcommand{\expeg}[1]{\underline{\mathbb{E}}_{Y_{\{#1\}}|\newinstance}\left[ \cdot \right]}
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, bottom color=blue!20},
  root/.style     = {treenode, font=\Large, bottom color=red!30},
  env/.style      = {treenode, font=\ttfamily\footnotesize},
  dummy/.style    = {circle,draw}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=4cm, sibling distance=2.7cm]
\tikzstyle{level 2}=[level distance=3.2cm, sibling distance=1.2cm]
% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [inner sep=0pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[
	grow=right, auto,
	sloped,
	edge from parent/.style = {draw, -latex, font=\tiny\sffamily, text=blue},
	every node/.style  = {font=\footnotesize}]
\node[root] {}
    child {
        node[env] {$y_1=1$}        
            child {
                node[end, label=right:{$(y_1\!=\!1, y_2\!=\!1)$}]  {}
                edge from parent
                node[below] (11) {$[0.613, \mathbf{0.713}]$}
            }
            child {
                node[end, label=right:{$(y_1\!=\!1, y_2\!=\!0)$}]  {}
                edge from parent
                node[above] (10) {$[\mathbf{0.287}, 0.387]$}
            }
            edge from parent 
            node[below] (1) {$[\mathbf{0.456}, 0.556]$} 
    }
    child {
        node[env] {$y_1=0$}       
        child {
                node[end, label=right:{$(y_1\!=\!0, y_2\!=\!1)$}] {}
                edge from parent
                node[below] (01) {$[0.138, \mathbf{0.238}]$}
            }
        child {
                node[end, label=right:{$(y_1\!=\!0, y_2\!=\!0)$}] {}
                edge from parent
                node[above] (00)  {$[\mathbf{0.762}, 0.862]$}
            }
        edge from parent         
        node[above] (0) {$[0.444, \mathbf{0.544}]$}
    };
\draw[red, transform canvas={xshift=-15pt}, bend right,-]  (11) to node [auto, yshift=-33pt, xshift=8pt] {\rotatebox{270}{$\lowerexp=0.287 \cdot 1$}} (10);

\draw[red, transform canvas={xshift=-15pt}, bend right,-]  (01) to node [auto,  yshift=-37pt, xshift=8pt] {\rotatebox{270}{$\lowerexp=0.238 \cdot -1$}} (00);

\draw[red, transform canvas={xshift=-15pt}, bend right,-]  (1) to node [auto, yshift=-87pt, xshift=8pt] {\rotatebox{270}{$\lowerexp=0.544 \cdot -0.238 + 0.456 \cdot 0.287 > 0$}} (0);

\node at (11,2.5) {$\ell_{0/1} \left((0,1),\cdot\right) - \ell_{0/1} \left((1,0),\cdot\right)= $};

\node at (11,1.95) {$0$};
\node at (11,0.75) {$-1$};
\node at (11,-0.75) {$1$};
\node at (11,-1.95) {$0$};
\end{tikzpicture}

==> resources/mlcbr/eg_precise_tree.tex <==
\newcommand{\exptwoeg}[3]{\underline{\mathbb{E}}_{Y_{\{#1\}}|\newinstance}\left[ \ell_H(\cdot, \overline{a}_\mathcal{I}) \middle| Y_{\{#2\}}\!=\!#3\right]}
\newcommand{\expeg}[1]{\underline{\mathbb{E}}_{Y_{\{#1\}}|\newinstance}\left[ \cdot \right]}
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, bottom color=blue!20},
  root/.style     = {treenode, font=\Large, bottom color=red!30},
  env/.style      = {treenode, font=\ttfamily\normalsize},
  dummy/.style    = {circle,draw}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=4cm, sibling distance=1.7cm]
\tikzstyle{level 2}=[level distance=3cm, sibling distance=0.8cm]
% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [inner sep=0pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%[0.444, 0.544] [0.456, 0.556]
%    00             01
%    [0.762, 0.862] [0.138, 0.238]
%    10             11
%    [0.287, 0.387] [0.613, 0.713]
\begin{tikzpicture}[
	grow=right, auto,
	sloped,
	edge from parent/.style = {draw, -latex, font=\tiny\sffamily, text=blue},
	every node/.style  = {font=\footnotesize}]
\node[root] {}
    child {
        node[env] {$y_1=1$}        
            child {
                node[end, label=right:{$(y_1\!=\!1, y_2\!=\!1)$}]  {}
                edge from parent
                node[below] (11) {$0.7$}
            }
            child {
                node[end, label=right:{$(y_1\!=\!1, y_2\!=\!0)$}]  {}
                edge from parent
                node[above] (10) {$0.3$}
            }
            edge from parent 
            node[below] (1) {$0.5$} 
    }
    child {
        node[env] {$y_1=0$}       
        child {
                node[end, label=right:{$(y_1\!=\!0, y_2\!=\!1)$}] {}
                edge from parent
                node[below] (01) {$0.2$}
            }
        child {
                node[end, label=right:{$(y_1\!=\!0, y_2\!=\!0)$}] {}
                edge from parent
                node[above] (00)  {$0.8$}
            }
        edge from parent         
        node[above] (0) {$0.5$}
    };
\end{tikzpicture}

==> resources/mlcbr/eg_prob_loss_tree.tex <==
\newcommand{\exptwoeg}[3]{\underline{\mathbb{E}}_{Y_{\{#1\}}|\newinstance}\left[ \ell_H(\cdot, \overline{a}_\mathcal{I}) \middle| Y_{\{#2\}}\!=\!#3\right]}
\newcommand{\expeg}[1]{\underline{\mathbb{E}}_{Y_{\{#1\}}|\newinstance}\left[ \cdot \right]}
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, bottom color=blue!20},
  root/.style     = {treenode, font=\Large, bottom color=red!30},
  env/.style      = {treenode, font=\ttfamily\footnotesize},
  dummy/.style    = {circle,draw}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=4cm, sibling distance=2.7cm]
\tikzstyle{level 2}=[level distance=3cm, sibling distance=1.2cm]
% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [inner sep=0pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[
	grow=right, auto,
	sloped,
	edge from parent/.style = {draw, -latex, font=\tiny\sffamily, text=blue},
	every node/.style  = {font=\footnotesize}]
\node[root] {}
    child {
        node[env] {$y_1=1$}        
            child {
                node[end, label=right:{$(y_1\!=\!1, y_2\!=\!1)$}]  {}
                edge from parent
                node[below] (11) {$0.7$}
            }
            child {
                node[end, label=right:{$(y_1\!=\!1, y_2\!=\!0)$}]  {}
                edge from parent
                node[above] (10) {$0.3$}
            }
            edge from parent 
            node[below] (1) {$0.5$} 
    }
    child {
        node[env] {$y_1=0$}       
        child {
                node[end, label=right:{$(y_1\!=\!0, y_2\!=\!1)$}] {}
                edge from parent
                node[below] (01) {$0.2$}
            }
        child {
                node[end, label=right:{$(y_1\!=\!0, y_2\!=\!0)$}] {}
                edge from parent
                node[above] (00)  {$0.8$}
            }
        edge from parent         
        node[above] (0) {$0.5$}
    };
\draw[red, bend right,-]  (11) to node [auto, yshift=-38pt, xshift=8pt] {\rotatebox{270}{$\expe_\prob=0.3 \cdot 1=0.3$}} (10);

\draw[red, bend right,-]  (01) to node [auto,  yshift=-46pt, xshift=8pt] {\rotatebox{270}{$\expe_\prob=0.2 \cdot -1=-0.2$}} (00);

\draw[red, bend right,-]  (1) to node [auto, yshift=69pt, xshift=8pt] {\rotatebox{90}{$\expe_\prob=0.5 \cdot -0.2 + 0.5 \cdot 0.3=0.05$}} (0);

\node at (11,2.5) {$\ell_{0/1} \left((0,1),\cdot\right) - \ell_{0/1} \left((1,0),\cdot\right)= $};

\node at (11,1.95) {$0$};
\node at (11,0.75) {$-1$};
\node at (11,-0.75) {$1$};
\node at (11,-1.95) {$0$};
\end{tikzpicture}

==> resources/mlcncc/marginalization_general_from.tex <==
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, 
                     bottom color=blue!20},
  root/.style     = {treenode, 
  		font=\Large, bottom color=black!30},
  one/.style      = {treenode, 
  		  minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
  		 shape=circle,
  		 bottom color=red!30,
  		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},
  zero/.style      = {treenode, 
  		 minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
		 shape=circle,
		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},	
  imprecise/.style      = {treenode, 
  		 minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
		 shape=circle,
		 bottom color=green!30,
		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},		 
  cross/.style={cross out, draw=black, solid, 
  	thick, minimum size=1.5*(#1-\pgflinewidth), 
  	inner sep=1.5, outer sep=0pt},
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 2}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 3}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 4}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 5}=[level distance=0.8cm, sibling distance=0.8cm]
% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [circle, minimum width=3pt,fill, inner sep=0pt]
\tikzstyle{pruned} = [cross, minimum width=3pt,fill, inner sep=0pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[
	grow=right, 
	sloped,
	edge from parent/.style = 
		{draw, font=\tiny\sffamily, text=blue},
	every node/.style = {font=\footnotesize}	]
\node(r)[root] {}
    child {
        node (1)[cross] {}        
        edge from parent 
        node[below] {}
    }
    child {
        node(2)[imprecise]{*}
        child {
            node(21)[one] {1}
            child {
            	node(211)[cross] {}
            }
            child {
        		node(212)[imprecise]{*}
        		child {
	              node(2121)[one,
	              		label=right:{\tred{\bf $(*, 1, *, ?)$}}] {1}    
	            }
	            child {
     			   node(2122)[cross]{}
			    }
	            child {
	              node(2120)[cross] {}
	            }
    		}
            child {
           		node(210)[cross]{}
            	edge from parent
            	node[above] {}
           }
        }
        child {
            node(02)[cross]{}
        }
        child {
            node(00)[cross]{}
            edge from parent
            node[above] {}
        }
        edge from parent         
        node[above] {}
    }
    child {
        node(0)[cross]{}
    };
\draw[dashed,->, bend left, red]  (r) to (2);
\draw[dashed,->, bend left, red] (2) to (21);
\draw[dashed,->, bend right, red] (21) to (212);
\draw[dashed,->, bend right, red] (212) to (2121);
\end{tikzpicture}







==> resources/mlcncc/marginalization_general_from_ncc.tex <==
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, 
                     bottom color=blue!20},
  root/.style     = {treenode, 
  		font=\Large, bottom color=black!30},
  one/.style      = {treenode, 
  		  minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
  		 shape=circle,
  		 bottom color=red!30,
  		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},
  zero/.style      = {treenode, 
  		 minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
		 shape=circle,
		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},	
  imprecise/.style      = {treenode, 
  		 minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
		 shape=circle,
		 bottom color=green!30,
		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},		 
  cross/.style={cross out, draw=black, solid, 
  	thick, minimum size=1.5*(#1-\pgflinewidth), 
  	inner sep=1.5, outer sep=0pt},
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=0.8cm, sibling distance=1.2cm]
\tikzstyle{level 2}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 3}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 4}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 5}=[level distance=0.8cm, sibling distance=0.8cm]
% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [circle, minimum width=3pt,fill, inner sep=0pt]
\tikzstyle{pruned} = [cross, minimum width=3pt,fill, inner sep=0pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[
	grow=right, 
	sloped,
	edge from parent/.style = 
		{draw, font=\tiny\sffamily, text=blue},
	every node/.style = {font=\footnotesize}	]
\node(r)[root] {}
    child {
        node(1)[one] {1}        
        child {
           node(11)[one, label=right:{\tred{\bf $(*, 1, *, ?)$}}] {1}
        }
        child {
        	node(12)[cross]{}
    	}
        child {
           node(10)[cross]{}
           edge from parent
           node[above] {}
        }
    }
    child {
        node(0)[cross] {}  
    };
\draw[dashed,->, bend left, red]  (r) to (1);
\draw[dashed,->, bend left, red] (1) to (11);
\node[yshift=12pt, xshift=1pt] at (1) {$Y_2$};
\node[yshift=-12pt, xshift=1pt] at (11) {$Y_4$};

\end{tikzpicture}






